Automated Synthesis of Asynchronizations

Asynchronous programming is widely adopted for building responsive and efficient software, and modern languages such as C# provide async/await primitives to simplify the use of asynchrony. In this paper, we propose an approach for refactoring a sequential program into an asynchronous program that uses async/await, called asynchronization. The refactoring process is parametrized by a set of methods to replace with asynchronous versions, and it is constrained to avoid introducing data races. We investigate the delay complexity of enumerating all data race free asynchronizations, which quantifies the delay between outputting two consecutive solutions. We show that this is polynomial time modulo an oracle for solving reachability in sequential programs. We also describe a pragmatic approach based on an interprocedural data-flow analysis with polynomial-time delay complexity. The latter approach has been implemented and evaluated on a number of non-trivial C# programs extracted from open-source repositories

==> preliminary-app.tex <==
%!TEX root = draft.tex

\section{Formalization of Section \ref{sec:1}}

\subsection{Syntax}\label{ssec:syntax}

Fig.~\ref{Figure:syntax} lists the syntax of a simple programming language used to formalize our approach.
% gives the syntax of our programming language. % syntax adopted from \cite{DBLP:conf/ecoop/BiermanRMMT12}. 
A \emph{program} is defined by set of methods, including a distinguished \texttt{main}, which are classified as \emph{synchronous} or \emph{asynchronous}.  
Synchronous methods execute immediately as they are invoked and run continuously until completion. 
Asynchronous methods, marked using the keyword \texttt{async}, can run only partially and be interrupted when executing an \texttt{await}. Only asynchronous methods are allowed to use \texttt{await}, and all methods using \texttt{await} must be defined as asynchronous. We assume that methods are not (mutually) recursive.
A program is called \emph{synchronous} if it is a set of synchronous methods. 

%whose names are taken from a set $\mathbb{M} = \ma \cup \ms$, where $\ma$ is for asynchronous methods and $\ms$ is for synchronous methods. 
A method consists of a method name from a set $\mathbb{M}$ and a method body, i.e., a list of statements. 
These statements use a set $\mathbb{PV}$ of \emph{program variables}, which can be accessed from different methods (ranged over using $x$, $y$, $z$,$\ldots$), and a set $\mathbb{LV}$ of method \emph{local variables} (ranged over using $r$, $r_1$, $r_2$,$\ldots$). 
%The  is used to declare a method as asynchronous .
 % and it is composed of a set of statements.
%starts with a \plog{begin} instruction, and finishes with an \plog{end} instruction. 
We assume that input/return parameters are modeled using dedicated program variables. We assume that each method call returns a \emph{unique task identifier} from a set $\mathbb{T}$, which is used to record control dependencies imposed by \plog{await}s (for uniformity, synchronous methods return a task identifier as well). 
Our language includes assignments to local/program variables, 
\plog{await}s, \plog{return} statements, \plog{while} loops, and conditionals. 
We assume that variables take values from a data domain $\mathbb{D}$, which includes $\mathbb{T}$ to account for variables storing task identifiers.
The assignment to a local variable $\langle r\rangle := \langle x\rangle$, where $x$ is a program variable, is called a \emph{read} of $\langle x\rangle$ and an assignment to a program variable $\langle x\rangle := \langle le\rangle$ is called a \emph{write} to $\langle x\rangle$. A \emph{base} method is a method whose body does \emph{not} contain method calls.

\begin{figure}[t]
%\vspace{-20pt}
{\footnotesize
\setlength{\grammarindent}{9em}
\setlength{\grammarparsep}{0.1cm}
\begin{grammar}
<prog> ::= \plog{program}  <md>

<md> ::= \plog{method} <m> <inst> |  \plog{async\ method} <m> <inst> | <md> ; <md>

<inst> ::=  <x> ":=" <le> | <r> ":=" <x> | <r> := \plog{call} <m> | \plog{return} | \plog{await} <r> | \plog{await} $*$ | \plog{if} <le> \{<inst>\} \plog{else} \{<inst>\} 
     \alt\plog{while} <le> \{<inst>\} | <inst> ; <inst>
\end{grammar}}
\vspace{-2mm}
\caption{Syntax. $\langle m\rangle$, $\langle x \rangle$, and $\langle r \rangle$ represent method names, program and local variables, resp. $\langle le \rangle$ is an expression over local variables, or $*$ which is non-deterministic choice.
}
\label{Figure:syntax}
\end{figure}

\begin{wrapfigure}{r}{0.59\textwidth}
  \vspace{-0.8cm}
  \lstset{basicstyle=\ttfamily\scriptsize,numbers=none,
            stepnumber=1,numberblanklines=false,mathescape=true,morekeywords={method,async,await}}
  \begin{minipage}[l]{0.323\linewidth}
  \begin{lstlisting}  
async method m {         
  while $*$
    r = call m1;

  await r;
}  
  \end{lstlisting}
  \end{minipage}
  \hfill
  \begin{minipage}{0.323\linewidth}
  \begin{lstlisting} 
async method m {   
  r = call m1; 

  if $*$
    await r;
} 
  \end{lstlisting}
  \end{minipage}
  \hfill
  \begin{minipage}[r]{0.323\linewidth}
  \begin{lstlisting} 
async method m { 
  r = call m1; 
  while $*$
    r' = call m1;
    await r';
  await r;   
} 
  \end{lstlisting}
  \end{minipage}
  \vspace{-0.7cm}
    \caption{Examples of programs} % (the code of $\ameth$ is irrelevant)
    \label{fig:synatactic-examples}
    \vspace{-0.4cm}
  \end{wrapfigure}
In Fig.~\ref{fig:synatactic-examples}, we give three examples of programs to explain in more details the well-formedness 
syntactic constraints. The program on the left of Fig.~\ref{fig:synatactic-examples} does not satisfy the second condition since \texttt{await} \texttt{r} can be reached without entering the loop. The program in the center of Fig.~\ref{fig:synatactic-examples} does not satisfy the third condition since we can reach the end of the method without entering the if branch and thus, without executing \texttt{await} \texttt{r}. The program on the right of Fig.~\ref{fig:synatactic-examples} satisfies both conditions. %The program on the right of Fig.~\ref{fig:synatactic-examples} satisfies both conditions.
\subsection{Semantics}\label{ssec:semApp}

A program configuration is a tuple $(\gsconf, \rtaskconf, \wtaskconf,\returnconf, \allowbreak \callrel, \awaitrel)$ where $\gsconf$ is composed of the valuation of the program variables excluding the program counter, % and the valuation of environment variables, e.g., files, 
$\rtaskconf$ is the call stack, $\wtaskconf$ is the set of asynchronous tasks, e.g., continuations predicated on the completion of some method call, $\returnconf$ is the set of completed tasks, $\callrel$ represents the relation between a method call and its caller, and $\awaitrel$ represents the control dependencies imposed by \plog{await} statements. 
%As expected, $\wtaskconf$ is empty in configurations of synchronous programs.
The activation frames in the call stack and the asynchronous tasks are represented using triples $(\aniden, \ameth,\lsconf)$ where $\aniden\in\mathbb{T}$ is a task identifier, $\ameth\in \mathbb{M}$ is a method name, and $\lsconf$ is a valuation of local variables, including as usual a dedicated program counter.
%and $\isIO$ is a boolean flag\footnote{We use $\top$ and $\bot$ to denote the true and false truth values.} set to true iff the task was interrupted by an \plog{await} $*$ statement.
The set of completed tasks is represented as a function $\returnconf:\mathbb{T}\rightarrow\{\top,\perp\}$ such that $\returnconf(\aniden)=\top$ when $\aniden$ is completed and $\returnconf(\aniden)=\perp$, otherwise.
We define $\callrel$ and $\awaitrel$ as partial functions $\mathbb{T}\rightharpoonup \mathbb{T}$ with the meaning that $\callrel(\aniden)=\anidenp$, resp., $\awaitrel(\aniden)=\anidenp$, iff $\aniden$ is called by $\anidenp$, resp., $\aniden$ is waiting for $\anidenp$. 
We set $\awaitrel(\aniden)=*$ if the task $\aniden$ was interrupted because of an $\mbox{\plog{await}}\ *$ statement. 

The semantics of a program $\aprog$ is defined as a labeled transition system (LTS) $[\aprog] =(\pstatesconf,\actionsconf,\psconf_0,\rightarrow)$ where $\pstatesconf$ is the set of program configurations, $\actionsconf$ is a set of transition labels called \emph{actions}, $\psconf_0$ is the initial configuration, and $\rightarrow\subseteq \pstatesconf\times \actionsconf\times \pstatesconf$ is the transition relation. Each program statement is interpreted as a transition in $[\aprog]$. The set of actions is defined by ($\actionsid$ is a set of action identifiers):
\vspace{-2mm}
\begin{align*}
  \actionsconf = & \{ (\actiden, \aniden, \event): \actiden \in \actionsid, \aniden \in \mathbb{T}, \event\in\{ \loadact(\anaddr), \storeact(\anaddr), \callact(\anidenp), \awaitact(\anidenk), \returnact,   \\ & \continueact: \anidenp \in \mathbb{T}, \anidenk \in \mathbb{T}\cup\{*\}, \anaddr\in \mathbb{PV}\}\} 
\vspace{-3mm}
\end{align*}

The transition relation $\rightarrow$ is defined in Fig.~\ref{Table:SemanticsRules}. Transition labels are written on top of $\rightarrow$. 
%\textcolor{red}{For a transition labeled by $(\actiden, \aniden, \event)$, $\actiden \in \actionsid$ is the unique identifier of the transition. We define the following mapping $\acttost$ that maps every action $\action$ in $\actionsconf \setminus \{ (\_, \_, \continueact)\}$ to a corresponding program statement $\acttost(\action) = \statement$.}  

Transitions labeled by $(\actiden, \aniden, \loadact(\anaddr))$ and $(\actiden, \aniden, \storeact(\anaddr))$ represent a read and a write accesses to the program variable $\anaddr$, respectively, executed by the task (method call) with identifier $\aniden$. 
%An $(\aniden, \loadact(\anaddr))$ transition reads the value of a program variable and stores it in a local variable, while an $(\aniden, \storeact(\anaddr))$ transition writes to a program variable $x$ the value of an expression over local variables.
%the value of a local variable and store it in .
A transition labeled by $(\actiden, \aniden, \callact(\anidenp))$ corresponds to the fact that task $\aniden$ executes a method call that results in creating a task $\anidenp$.
% a method call executed by the task with id $\aniden$  that creates another  task with the  unique id $\anidenp$ from the set $\mathbb{T}$.
Task $\anidenp$ is added on the top of the stack of currently executing tasks, declared pending (setting $\returnconf(j)$ to $\perp$), and $\callrel$ is updated to track its caller ($\callrel(\anidenp)=\aniden$).
%We assume that calls to synchronous method are aligned. Thus, in our semantics we don't consider synchronous calls.
A transition $(\actiden, \aniden, \returnact)$ represents the return from task $\aniden$.
Task $\aniden$ is removed from the stack of currently executing tasks, and $\returnconf(\aniden)$ is set to $\top$ to record the fact that task $\aniden$ is finished.

A transition $(\actiden, \aniden, \awaitact(\anidenp))$ relates to task $\aniden$ waiting asynchronously for task $\anidenp$. Its effect depends on whether task $\anidenp$ is already completed. If this is the case (i.e., $\returnconf[\anidenp]=\top$), task $\aniden$ continues and executes the next statement.
%% in the task with id $\aniden$ for the return of the task identified by $\anidenp$.
%Its corresponding transition will try to wait for the result of the task $\anidenp$ and when the task $\anidenp$ is already finished and its result is ready (i.e., $\returnconf[\anidenp]$  is equal to $\top$), the task executing the transition continues and executes the next statement. 
Otherwise, task $\aniden$ executing the $\awaitact$ is removed from the stack and added to the set of pending tasks, and $\awaitrel$ is updated to track the waiting-for relationship ($\awaitrel(\aniden)=\anidenp$). 
%Updating $\awaitrel$ signals that the task with the identifier $\aniden$ is waiting for the return of the task with the identifier $\anidenp$.
Similarly, a transition $(\actiden, \aniden, \awaitact(*))$ corresponds to task $\aniden$ waiting asynchronously for the completion of an unspecified task. Non-deterministically, task $\aniden$ continues to the next statement, or task $\aniden$ is interrupted and transferred to the set of pending tasks ($\awaitrel(\aniden)$ is set to $*$).

A transition $(\actiden, \aniden, \continueact)$ represents the scheduling of the continuation of task $\aniden$. There are two cases depending on whether $\aniden$ waited for the completion of another task $\anidenp$ modeled explicitly in the language (i.e., $\awaitrel(\aniden)=\anidenp$), or an unspecified task (i.e., $\awaitrel(\aniden)=*$). In the first case, the transition is enabled only when the call stack is empty and $\anidenp$ is completed. In the second case, the transition is always enabled. The latter models the fact that methods implementing IO operations (waiting for unspecified tasks in our language) are executed in background threads and can interleave with the main thread (that executes the \texttt{Main} method). Although this may seem restricted because we do not allow arbitrary interleavings between such methods, this is actually sound when focusing on the existence of data races as in our approach. As shown later in Table~\ref{Table:TracesOrders}, any two instructions that follow an \plog{await} $*$ are not happens-before related and form a race.

By the definition of the transition relation $\rightarrow$, every action $\action\in \actionsconf \setminus \{ (\_, \_, \continueact)\}$ corresponds to executing some statement in the program, which is denoted by $\acttost(a)$.


\begin{figure}[!t]
  \small\addtolength{\tabcolsep}{-5pt}
  \therules{
  \scriptsize
  \therule
  {$\text{\plog{\theload{\areg}{\anaddr}}}\in\instrOf(\lsconf(\pcconf))$\quad
  $\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\lsconf' = \lsconf[\areg \mapsto \gsconf(\anaddr),\pcconf\mapsto \mathsf{next}(\lsconf(\pcconf))]$}
  {$(\gsconf, (\aniden,\ameth,\lsconf) \circ \rtaskconf, \_, \_, \_, \_)
  \mpitrans{(\actiden, \aniden, \loadact(\anaddr))}
   (\gsconf, (\aniden,\ameth,\lsconf') \circ \rtaskconf, \_, \_, \_, \_)$}
  \scriptsize
  \therule
  {$\text{\plog{\thestore{\anaddr}{le}}}\in\instrOf(\lsconf(\pcconf))$\quad
  $\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\lsconf' = \lsconf[\pcconf\mapsto \mathsf{next}(\lsconf(\pcconf))]$ \quad
  $\gsconf' = \gsconf[\anaddr \mapsto \lsconf(\text{\plog{le}})]$}
  {$(\gsconf, (\aniden,\ameth,\lsconf) \circ \rtaskconf, \_, \_, \_, \_)
  \mpitrans{(\actiden, \aniden, \storeact(\anaddr))}
  (\gsconf', (\aniden,\ameth,\lsconf') \circ \rtaskconf, \_, \_, \_, \_)$}
  \scriptsize
  %\therule
  \dfrac
  {\splitdfrac{\text{$\theassign{\areg}{\callact\ \ameth}\in\instrOf(\lsconf(\pcconf))$\quad
  $\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\ell_0 = \mathsf{init}(\gsconf,\ameth)$ \quad
  $\anidenp\in\mathbb{T}$ fresh  }}% \quad
  {\text{$\ell' = \lsconf[\areg\mapsto\anidenp,\pcconf\mapsto \mathsf{next}(\lsconf(\pcconf))]$ \quad 
  $\returnconf' = \returnconf[\anidenp \mapsto \perp]$ \quad $\callrel' = \callrel[\anidenp \mapsto \aniden]$}}}
  {\text{$(\gsconf, (\anidenp, \ameth',\lsconf) \circ \rtaskconf, \_, \returnconf, \callrel, \_)
  \mpitrans{(\actiden, \aniden, \callact(\anidenp))}
  (\gsconf, (\aniden,\ameth,\lsconf_0) \circ (\anidenp,\ameth',\ell') \circ \rtaskconf, \_, \returnconf', \callrel', \_)$}}
  \\[1.5em]
  \scriptsize
  \therule
  {$\text{\plog{\returnact}}\in\instrOf(\lsconf(\pcconf))$ \quad
  $\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\returnconf' = \returnconf[\aniden \mapsto \top]$}
  {$(\gsconf, (\aniden, \ameth,\lsconf) \circ \rtaskconf, \_, \returnconf, \_, \_)
  \mpitrans{(\actiden, \aniden, \returnact)}
  (\gsconf, \rtaskconf, \_, \returnconf', \_, \_)$}
  \scriptsize
  \therule
  {$\text{\plog{\awaitact\ \areg}}\in\instrOf(\lsconf(\pcconf))$ \quad
  $\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\returnconf(\lsconf(\areg)) = \top$ \quad
  $\lsconf' = \lsconf[\pcconf\mapsto \mathsf{next}(\lsconf(\pcconf))]$ }
  {$(\gsconf, (\aniden, \ameth,\lsconf) \circ \rtaskconf, \_, \returnconf, \_, \_)
  \mpitrans{(\actiden, \aniden, \awaitact(\lsconf(\areg)))}
  (\gsconf, (\aniden, \ameth, \lsconf') \circ \rtaskconf, \_, \returnconf, \_, \_)$}
  \scriptsize
  \therule
  {$\text{\plog{\awaitact\ \areg}}\in\instrOf(\lsconf(\pcconf))$ \quad
  $\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\returnconf(\lsconf(\areg)) = \perp$ \quad
  $\awaitrel' = \awaitrel[\aniden \mapsto \lsconf(\areg)]$ \quad
  $\lsconf' = \lsconf[\pcconf\mapsto \mathsf{next}(\lsconf(\pcconf))]$}
  {$(\gsconf, (\aniden, \ameth,\lsconf) \circ \rtaskconf, \wtaskconf, \returnconf, \_, \awaitrel)
  \mpitrans{(\actiden, \aniden, \awaitact(\lsconf(\areg)))}
  (\gsconf, \rtaskconf, \{(\aniden, \ameth,\lsconf')\} \uplus \wtaskconf, \returnconf, \_, \awaitrel')$}
  \scriptsize
  \therule
  {$\text{\plog{\awaitact\ *}}\in\instrOf(\lsconf(\pcconf))$ \quad
  $\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\lsconf' = \lsconf[\pcconf\mapsto \mathsf{next}(\lsconf(\pcconf))]$ }
  {$(\gsconf, (\aniden, \ameth,\lsconf) \circ \rtaskconf, \_, \_, \_, \_)
  \mpitrans{(\actiden, \aniden, \awaitact(*))}
  (\gsconf, (\aniden, \ameth, \lsconf') \circ \rtaskconf, \_, \_, \_, \_)$}
  \scriptsize
  \therule
  {$\text{\plog{\awaitact\ *}}\in\instrOf(\lsconf(\pcconf))$ \quad
  $\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\awaitrel' = \awaitrel[\aniden \mapsto \ *]$ \quad
  $\lsconf' = \lsconf[\pcconf\mapsto \mathsf{next}(\lsconf(\pcconf))]$}
  {$(\gsconf, (\aniden, \ameth,\lsconf) \circ \rtaskconf, \wtaskconf, \_, \_, \awaitrel)
  \mpitrans{(\actiden, \aniden, \awaitact(*))}
  (\gsconf, \rtaskconf, \{(\aniden, \ameth,\lsconf')\} \uplus \wtaskconf, \_, \_, \awaitrel')$}
  \scriptsize
  \therule
  {$\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\awaitrel(\aniden) = \anidenp$ \quad
  $\returnconf(\anidenp) = \top$
  }
  {$(\gsconf, \epsilon, \{(\aniden, \ameth,\lsconf)\} \uplus \wtaskconf, \returnconf, \_, \awaitrel)
  \mpitrans{(\actiden, \aniden, \continueact)}
  (\gsconf,  (\aniden, \ameth,\lsconf) ,  \wtaskconf, \returnconf, \_,  \awaitrel)$}
  \scriptsize
  \therule
  {$\actiden\in\mathbb{\actionsid}$ fresh \quad 
  $\awaitrel(\aniden) = *$
  }
  {$(\gsconf, \rtaskconf, \{(\aniden, \ameth,\lsconf)\} \uplus \wtaskconf, \_, \_, \awaitrel)
  \mpitrans{(\actiden, \aniden, \continueact)}
  (\gsconf,  (\aniden, \ameth,\lsconf) \circ \rtaskconf,  \wtaskconf, \_, \_,  \awaitrel)$}
  }
  \vspace{-0.6cm}
  \caption{Program semantics. For a function $f$, we use $f[a\mapsto b]$ to denote a function $g$ such that $g(c)=f(c)$ for all $c\neq a$ and $g(a)=b$. The function $\instrOf$ returns the instruction at some given control location while $\mathsf{next}$ gives the next instruction to execute. We use $\circ$ to denote sequence concatenation. We use $\mathsf{init}$ to represent the initial state of a method call.
  }
  \label{Table:SemanticsRules}
  \end{figure}

  An execution of $\aprog$ is a sequence $\rho=\psconf_0\xrightarrow{\action_1}\psconf_1\xrightarrow{\action_2}\ldots$ of transitions starting in the initial configuration $\psconf_0$
  and leading to a configuration $\psconf$ where the call stack and the set of pending tasks are empty. 
   $\pstatesconf[\aprog]$ denotes the set of all program variable valuations included in configurations that are reached in executions of $\aprog$.
  % to a configuration $\psconf \in \pstatesconf[\aprog]$. 
  Since we are only interested in reasoning about the sequence of actions $\action_1\cdot\action_2\cdot\ldots$ labeling the transitions of an execution, we will call the latter an execution as well. The set of executions of a program $\aprog$ is denoted by $\executionsconf(\aprog)$. 
  
  %\vspace{1mm}
  \noindent
  {\bf Traces.} 
  %We define the notion of \emph{trace} which is an abstract representation of an execution. 
  The \emph{trace} of an execution $\rho \in \executionsconf(\aprog)$ is a tuple $\traceof{\rho} = (\rho, \mo{}, \co{}, \so{}, \hbo{})$ of strict partial orders between the actions in $\rho$ defined in Table \ref{Table:TracesOrders}. The \emph{method invocation order} $\mo$ records the order between actions in the same invocation, and the \emph{call order} $\co$ is an extension of $\mo$ that additionally orders actions before an invocation with respect to those inside that invocation. The \emph{synchronous happens-before order} $\so$ orders the actions in an execution as if all the invocations were synchronous (even if the execution may contain asynchronous ones). It is an extension of $\co$ where additionally, every action inside a callee is ordered before the actions following its invocation in the caller. The (asynchronous) \emph{happens-before order} $\hbo{}$ contains typical control-flow constraints: it is an extension of $\co$ where every action $a$ inside an asynchronous invocation is ordered before the corresponding $\mathtt{await}$ in the caller, and before the actions following its invocation in the caller if $a$ precedes the first\footnote{Code in between two awaits can execute before or after the control is returned to the caller, depending on whether the first awaited task finished or not.} $\mathtt{await}$ in $\mo$ (an invocation can be interrupted only when executing an $\mathtt{await}$) or if the callee does not contain an $\mathtt{await}$ (it is  synchronous).
  %Fig. \ref{fig:execution3} shows a trace where two statements are linked by a dotted arrow if the corresponding actions are related by $\mo$, a dashed arrow if the corresponding actions are related by the $\co$ but not by $\mo$, and a solid arrow if the corresponding actions are related by the $\hbo{}$ but not by $\co$. 
  $\tracesconf(\aprog)$ is the set of traces of $\aprog$. 
  

  \begin{table}
    \caption{Strict partial orders included in a trace.} \label{Table:TracesOrders}
    \vspace{-0mm}
  {\footnotesize
  \begin{tabular}{|c|c|}
    \hline
    $\action_1 <_{\rho} \action_2$ & $\action_1$ occurs before  $\action_2$ in $\rho$ and $\action_1 \neq \action_2$\\[.5mm] \hline
    $\action_1 \sim \action_2$ & $\action_1=(\_,\aniden, \event)$ and $\action_2=(\_,\aniden, \event')$ \\[.5mm] \hline
    \hline
    $(\action_1,\action_2) \in \mo{}$ & $\action_1 \sim \action_2 \wedge \action_1 <_{\rho} \action_2$ \\ \hline
    $(\action_1,\action_2) \in \co{}$ & $(\action_1,\action_2) \in \mo{} \vee (\action_1 = (\_,\aniden, \callact(\anidenp)) \wedge \action_2 = (\_,\anidenp,\_))$ \\
    & $\vee\ (\exists\ \action_3.\  (\action_1,\action_3) \in \co{} \wedge (\action_3,\action_2) \in \co{})$ \\[.5mm]\hline
    $(\action_1,\action_2) \in \so{}$ & $(\action_1,\action_2) \in \co{} \vee (\exists\ \action_3.\  (\action_1,\action_3) \in \so{} \wedge (\action_3,\action_2) \in \so{})$ \\
    & $\vee\ (\action_1 = (\_,\anidenp, \_) \wedge \action_2 = (\_,\aniden,\_) \wedge \exists\ \action_3 = (\_,\aniden, \callact(\anidenp)).\ \action_3 <_{\rho} \action_2)$ \\[.5mm]\hline
    $(\action_1,\action_2) \in \hbo{}$  & $(\action_1,\action_2) \in \co{} \vee (\exists\ \action_3.\  (\action_1,\action_3) \in \hbo{} \wedge (\action_3,\action_2) \in \hbo{})$ \\ 
     & $\vee\ (\action_1 = (\_,\anidenp, \_) \wedge \action_2 = (\_,\aniden,\_) \wedge \exists\ \action_3 = (\_,\aniden, \awaitact(\anidenp)).\ \action_3 <_{\rho} \action_2 )$ \\
     \cline{1-1}\multicolumn{2}{|c|}{ $\vee\ (\action_1 = (\_, \anidenp, \awaitact(\aniden'))$ is the first await in $\anidenp \wedge \action_2 = (\_,\aniden,\_)  \wedge \exists\ \action_3 = (\_,\aniden, \callact(\anidenp)).\ \action_3 <_{\rho} \action_2)$} \\
    \multicolumn{2}{|c|}{ $\vee\ (\action_1 = (\_, \anidenp, \_)\ \wedge \not\exists\ (\_, \anidenp, \awaitact(\_)) \in\rho \wedge \action_2 = (\_,\aniden,\_)  \wedge \exists\ \action_3 = (\_,\aniden, \callact(\anidenp)).\ \action_3 <_{\rho} \action_2)$} \\ [.5mm]\hline
  \end{tabular}}
  \end{table}

  






